VLASE: Vehicle Localization by Aggregating Semantic Edges

In this paper, we propose VLASE, a framework to use semantic edge features from images to achieve on-road localization. Semantic edge features denote edge contours that separate pairs of distinct objects such as building-sky, road- sidewalk, and building-ground. While prior work has shown promising results by utilizing the boundary between prominent classes such as sky and building using skylines, we generalize this approach to consider semantic edge features that arise from 19 different classes. Our localization algorithm is simple, yet very powerful. We extract semantic edge features using a recently introduced CASENet architecture and utilize VLAD framework to perform image retrieval. Our experiments show that we achieve improvement over some of the state-of-the-art localization algorithms such as SIFT-VLAD and its deep variant NetVLAD. We use ablation study to study the importance of different semantic classes and show that our unified approach achieves better performance compared to individual prominent features such as skylines.

==> analysis.tex <==
\section{Analysis}

- For SLC Data, removing dynamic classes yields better accuracy than all classes. E.g. removing car improves accuracy by 2%, removing truck improves accuracy by 1.5% \\

- For KAIST, removal of some dynamic classes causes drop in accuracy. E.g. removing truck and bus cause 1% drop. It may be because these dynamic objects are actually static in the videos as they may be parked in both the sequences of KAIST dataset \\

- Using only static classes of casenet performs better than using all classes, for both datasets \\

- For SLC Data, building, sky and wall are the top 3 individual contributors as removing them causes highest drop in the accuracy \\

- For SLC Data, using only vegetation and sky performs really close to using all static classes; in case of Top 1 neighbor, it has better accuracy than all static classes \\

- SIFT features perform better on KAIST data than on SLC dataset, even with x,y coordinates. The reason can be lower frame rate of KAIST data videos which provides SIFT with more discriminative keypoints in lesser distance. \\

- SIFT without x,y has very low accuracy on SLC data and the reason can be higher frame rate of SLC Data. \\

- For KAIST, top 1 accuracies of SIFT with x,y are better tha casenet but casenet has better top 5 accuracies. As the distance threshold increases from 1 to 20 meters, casenet accuracies get better than SIFT. \\

- 


